Towards Causal Representation Learning with Observable Sources as Auxiliaries

Causal representation learning seeks to recover latent factors that generate observational data through a mixing function. Needing assumptions on latent structures or relationships to achieve identifiability in general, prior works often build upon conditional independence given known auxiliary variables. However, prior frameworks limit the scope of auxiliary variables to be external to the mixing function. Yet, in some cases, system-driving latent factors can be easily observed or extracted from data, possibly facilitating identification. In this paper, we introduce a framework of observable sources being auxiliaries, serving as effective conditioning variables. Our main results show that one can identify entire latent variables up to subspace-wise transformations and permutations using volume-preserving encoders. Moreover, when multiple known auxiliary variables are available, we offer a variable-selection scheme to choose those that maximize recoverability of the latent factors given knowledge of the latent causal graph. Finally, we demonstrate the effectiveness of our framework through experiments on synthetic graph and image data, thereby extending the boundaries of current approaches.

==> algorithm/alg2_gfc.tex <==
\begin{algorithm}[t]
    \begin{algorithmic}[1]
    \STATE \textbf{Input}: graph $G=(\*V, \*E)$, condition $C$, observed set $O$
    \STATE \textbf{Output}: a set of d-connected node clusters $R$
    \STATE $R \gets \emptyset$

    \FOR{each node $n$ in $\*V\setminus O$}
 \IF{$\exists_{\*C\in R}\, n \in \*C$}
            \STATE continue
        \ENDIF
        \STATE $result \gets \{n\}$;  %$prev\_result \gets \emptyset$
        %\WHILE{$prev\_result \neq result$}  
        %\Comment{Repeat until no change in result}
        \WHILE{$result$ updated}
            %\STATE $prev\_result \gets result$
            \STATE $result \gets$ \textsc{BayesBall}$(G, C, O, result)$
        \ENDWHILE
        \STATE Add $result$ to $R$
    \ENDFOR
    
    \STATE \textbf{return} $R$
 %    \STATE Initialize $R$ as an empty set for storing clusters

 %    \FOR{each node $n$ in $G$}
 % \IF{n $\in R$ or n $\in O$}
 %            \STATE continue
 %        \ENDIF
 %        \STATE Initialize $result \gets \{n\}$
 %        \STATE Initialize $prev\_result$ as an empty set
        
 %        \WHILE{$prev\_result \neq result$}  %\Comment{Repeat until no change in result}
 %            \STATE $prev\_result \gets result$
 %            \STATE $result \gets$ \textsc{BayesBall}$(G, C, O, result)$
 %        \ENDWHILE
        
 %        \STATE Add $result$ to $R$
 %    \ENDFOR
    
 %    \STATE \textbf{return} $R$
    \end{algorithmic}
\caption{Graph Partition by Conditional Independence}\label{alg:iterative_bayes_ball}
\end{algorithm}

==> figs/fig1.tex <==
\begin{figure}[t]\centering
\begin{subfigure}[b]{0.15\textwidth}\centering
\captionsetup{justification=centering}
    \begin{tikzpicture}[x=.8cm,y=8mm,scale=0.75,transform shape,font=\normalsize]
% 첫 번째 그래프
\node[RR, minimum size=7mm][fill=betterblue!50] (u1) at (0, 2) {$u$};
\node[RR, minimum size=7mm] (z1) at (-1.5, 0) {$z_1$};
\node[RR, minimum size=7mm] (z2) at (-0.5, 0) {$z_2$};
\node[RR, minimum size=7mm] (z3) at (0.5, 0) {$z_3$};
\node[RR, minimum size=7mm] (z5) at (1.5, 0) {$z_5$};
% \node[RR, minimum size=7mm][fill=betterblue] (x) at (0, -2) {$x$};

\draw[->] (u1) -- (z1);
\draw[->] (u1) -- (z2);
\draw[->] (u1) -- (z3);
\draw[->] (u1) -- (z5);
% \draw[->] (s1) -- (x);
% \draw[->] (s2) -- (x);
% \draw[->] (s3) -- (x);
\end{tikzpicture}
\caption{}
\label{fig1:graph_a}
\end{subfigure}
% 두 번째 그래프
\begin{subfigure}[b]{0.15\textwidth}\centering
\captionsetup{justification=centering}
    \begin{tikzpicture}[x=.8cm,y=8mm,scale=0.75,transform shape,font=\normalsize]
\node[RR, minimum size=7mm] (u1_c) at (8, 2) {$z_3$};
\node[RR, minimum size=7mm] (z1_c) at (6.5, 0) {$z_1$};
\node[RR, minimum size=7mm][fill=betterblue!50] (z2_c) at (8, 0) {$z_5$};
\node[RR, minimum size=7mm] (z3_c) at (9.5, 0) {$z_4$};
\node[RR, minimum size=7mm] (z5_c) at (6.5, 2) {$z_2$};
% \node[RR, minimum size=7mm][fill=betterblue] (x_c) at (8, -2) {$x$};

\draw[->] (u1_c) -- (z2_c);
\draw[->] (u1_c) -- (z3_c);
% \draw[->] (s1_c) -- (x_c);
% \draw[->] (s2_c) -- (x_c);
% \draw[->] (s3_c) -- (x_c);
\draw[->] (z2_c) -- (z1_c);
\draw[->] (z2_c) -- (z3_c);
\draw[->] (z2_c) -- (z5_c);
\end{tikzpicture}
\caption{}
\label{fig2:graph_b}
\end{subfigure}
% 세 번째 그래프
\begin{subfigure}[b]{0.15\textwidth}\centering
    \begin{tikzpicture}[x=.8cm,y=8mm,scale=0.75,transform shape,font=\normalsize]
\node[RR, minimum size=7mm][fill=betterblue!50] (z4_c) at (8, 2) {$z_4$};
\node[RR, minimum size=7mm] (z1_c) at (6.5, 0) {$z_1$};
\node[RR, minimum size=7mm][fill=betterblue!50] (z2_c) at (8, 0) {$z_2$};
\node[RR, minimum size=7mm] (z3_c) at (9.5, 0) {$z_3$};
% \node[RR, minimum size=7mm][fill=betterblue] (x_c) at (8, -2) {$x$};

% \draw[->] (s4_c) -- (s2_c);
\draw[->] (z4_c) -- (z3_c);
\draw[->] (z1_c) -- (u1_c);
% \draw[->] (s2_c) -- (x_c);
% \draw[->] (s3_c) -- (x_c);
\draw[<-] (z2_c) -- (z1_c);
\draw[<-] (z2_c) -- (z3_c);
\end{tikzpicture}
\caption{}
\label{fig3:graph_c}
\end{subfigure}
\caption{Examples of data generating process except mixing process, i.e. latent mechanism. Blue nodes represent the observable variables.}
\label{fig1}
\end{figure}

==> proposition/proposition-aux.tex <==


\begin{proposition}\label{prop:auxiliary}
    Suppose the following assumptions hold:
    \begin{enumerate}
        \item The observed data and sources are generated from \Cref{eqn1:generation} and \Cref{eqn4:cond_indep_observed}
        \item The observable sources do not have direct edge into the observation $\rvx$, i.e., $\frac{\partial \rvx}{\partial \rvz_o} = 0$
        \item For every value of $\rvz_D$, there exists $2d+1$ values of $\rvz_o$,
        % There exist $2d+1$ values of $\rvz_o$, i.e. $\rvz_{o_i}$ with $i \in \{0,1,\dots,2d\}$, 
        such that the $2d$ vectors $\rvw(\rvz_D, \rvz_{o_i}) - \rvw(\rvz_D, \rvz_{o_0})$ are linearly independent, where vector $\rvw(Z_D, \rvz_{o_i})$ is defined as follows:
        \begin{align*}
            \rvw(\rvz_D, \rvz_{o_i}) &= \big( \rvv(\rvz_{c_1}, \rvz_{o_i}), \dots, \rvv(\rvz_{c_d}, \rvz_{o_i}), \\
            &\quad \rvv'(\rvz_{c_1}, \rvz_{o_i}), \dots, \rvv'(\rvz_{c_d}, \rvz_{o_i}) \big)
        \end{align*}
        where
        \begin{align*}
        \rvv(\rvz_{c_j}, \rvz_{o_i}) &= \left( \frac{\partial \log p(\rvz_{c_j} \mid \rvz_{o_i})}{\partial z_{c_j}^{(l)}}, \dots, \frac{\partial \log p(\rvz_{c_j} \mid \rvz_{o_i})}{\partial z_{c_j}^{(h)}} \right), \\
        \rvv'(\rvz_{c_j}, \rvz_{o_i}) &= \left( \frac{\partial^2 \log p(\rvz_{c_j} \mid \rvz_{o_i})}{\partial (z_{c_j}^{(l)})^2}, \dots, \frac{\partial^2 \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial (z_{c_j}^{(h)})^2} \right)
        \end{align*} and $\rvz_{c_j} = (z_{c_{j}^{(l)}},\dots,z_{c_{j}^{(h)}})$.
    \end{enumerate}
    Then all components of $\rvz_D$ (i.e., $\rvz_{c_i}$ where $c_i \in \{c_1,\dots,c_d\}$) is identifiable up to a subspace-wise invertible transformation and a subspace-wise permutation.
\end{proposition}

==> proposition/proposition-partial-aaai.tex <==
\begin{proposition}\label{prop:partial}
    Suppose the following assumptions hold:
    %\begin{enumerate}
        1. The observed data and sources are generated from \ref{eqn1:generation} and \ref{eqn4:cond_indep_observed}
        
        2. The mixing function $g$ is volume-preserving, i.e., $|\text{det}(\mathbf{J}_g(\rvz))| = 1$
        
        3. For every value of $\rvz_{o^-}$, there exists $2d$ values of $\rvz_o$,
        % There exist $2d$ values of $\rvz_o$, i.e. $\rvz_{o_i}$ with $i \in \{0,1,\dots,2d-1\}$, 
         such that the $2d$ vectors $\rvw(\rvz_{o^-}, \rvz_{o_i})$ are linearly independent, where vector $\rvw(\rvz_{o^-}, \rvz_{o_i})$ is defined as follows:
        \begin{align*}
        \rvw(\rvz_{o^-}, \rvz_{o_i}) = \big( &\rvv(\rvz_{c_1}, \rvz_{o_i}), \dots, \rvv(\rvz_{c_d}, \rvz_{o_i}), \\
            &\rvv'(\rvz_{c_1}, \rvz_{o_i}), \dots, \rvv'(\rvz_{c_d}, \rvz_{o_i}) \big)
        \end{align*}
    %\end{enumerate}
    where {\footnotesize
        \begin{align*}
        \rvv(\rvz_{c_j}, \rvz_{o_i}) &= \left(\! \frac{\partial \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial z_{c_j}^{(l)}}, \dots, \frac{\partial \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial z_{c_j}^{(h)}} \!\right), \\
        \rvv'(\rvz_{c_j}, \rvz_{o_i}) &= \left(\! \frac{\partial^2\! \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial (z_{c_j}^{(l)})^2},  \dots, \frac{\partial^2\! \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial (z_{c_j}^{(h)})^2} \!\right)
        \end{align*}} and $\rvz_{c_j} = (z_{c_{j}^{(l)}},\dots,z_{c_{j}^{(h)}})$.

    Then all the components of $\rvz_{o^-}$ (i.e., $\rvz_{c_i}$ where $c_i \in \{c_1,\dots,c_d\}$) is identifiable up to a subspace-wise invertible transformation and a subspace-wise permutation.
\end{proposition}

==> proposition/proposition-partial-uai.tex <==
\begin{proposition}\label{prop:partial}
    Suppose the following assumptions hold:
    \begin{enumerate}
        \item The observed data and sources are generated from \Cref{eqn1:generation} and \Cref{eqn4:cond_indep_observed}
        
        \item The mixing function $g$ is volume-preserving, i.e., $|\text{det}(\mathbf{J}_g(\rvz))| = 1$
        
        \item For every value of $\rvz_{o^-}$, there exists $2d$ values of $\rvz_o$,
        % There exist $2d$ values of $\rvz_o$, i.e. $\rvz_{o_i}$ with $i \in \{0,1,\dots,2d-1\}$, 
         such that the $2d$ vectors $\rvw(\rvz_{o^-}, \rvz_{o_i})$ are linearly independent, where vector $\rvw(\rvz_{o^-}, \rvz_{o_i})$ is defined as follows:
        \begin{align*}
        \rvw(\rvz_{o^-}, \rvz_{o_i}) &= \big( \rvv(\rvz_{c_1}, \rvz_{o_i}), \dots, \rvv(\rvz_{c_d}, \rvz_{o_i}), \\
            &\quad \rvv'(\rvz_{c_1}, \rvz_{o_i}), \dots, \rvv'(\rvz_{c_d}, \rvz_{o_i}) \big)
        \end{align*}
    \end{enumerate}
    where {\footnotesize
        \begin{align*}
        \rvv(\rvz_{c_j}, \rvz_{o_i}) &= \left(\! \frac{\partial \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial z_{c_j}^{(l)}}, \dots, \frac{\partial \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial z_{c_j}^{(h)}} \!\right), \\
        \rvv'(\rvz_{c_j}, \rvz_{o_i}) &= \left(\! \frac{\partial^2\! \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial (z_{c_j}^{(l)})^2},  \dots, \frac{\partial^2\! \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial (z_{c_j}^{(h)})^2} \!\right)
        \end{align*}} and $\rvz_{c_j} = (z_{c_{j}^{(l)}},\dots,z_{c_{j}^{(h)}})$.

    Then all the components of $\rvz_{o^-}$ (i.e., $\rvz_{c_i}$ where $c_i \in \{c_1,\dots,c_d\}$) is identifiable up to a subspace-wise invertible transformation and a subspace-wise permutation.
\end{proposition}

==> proposition/proposition-partial.tex <==
\begin{proposition}\label{prop:partial}
    Suppose the following assumptions hold:
    %\begin{enumerate}
        1. The observed data and sources are generated from \Cref{eqn1:generation} and \Cref{eqn4:cond_indep_observed}
        
        2. The mixing function $g$ is volume-preserving, i.e., $|\text{det}(\mathbf{J}_g(\rvz))| = 1$
        
        3. For every value of $\rvz_{o^-}$, there exists $2d$ values of $\rvz_o$,
        % There exist $2d$ values of $\rvz_o$, i.e. $\rvz_{o_i}$ with $i \in \{0,1,\dots,2d-1\}$, 
         such that the $2d$ vectors $\rvw(\rvz_{o^-}, \rvz_{o_i})$ are linearly independent, where vector $\rvw(\rvz_{o^-}, \rvz_{o_i})$ is defined as follows:
        \begin{align*}
        \rvw(\rvz_{o^-}, \rvz_{o_i}) &= \big( \rvv(\rvz_{c_1}, \rvz_{o_i}), \dots, \rvv(\rvz_{c_d}, \rvz_{o_i}), \\
            &\quad \rvv'(\rvz_{c_1}, \rvz_{o_i}), \dots, \rvv'(\rvz_{c_d}, \rvz_{o_i}) \big)
        \end{align*}
    %\end{enumerate}
    where {\footnotesize
        \begin{align*}
        \rvv(\rvz_{c_j}, \rvz_{o_i}) &= \left(\! \frac{\partial \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial z_{c_j}^{(l)}}, \dots, \frac{\partial \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial z_{c_j}^{(h)}} \!\right), \\
        \rvv'(\rvz_{c_j}, \rvz_{o_i}) &= \left(\! \frac{\partial^2\! \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial (z_{c_j}^{(l)})^2},  \dots, \frac{\partial^2\! \log p(\rvz_{c_j} | \rvz_{o_i})}{\partial (z_{c_j}^{(h)})^2} \!\right)
        \end{align*}} and $\rvz_{c_j} = (z_{c_{j}^{(l)}},\dots,z_{c_{j}^{(h)}})$.

    Then all the components of $\rvz_{o^-}$ (i.e., $\rvz_{c_i}$ where $c_i \in \{c_1,\dots,c_d\}$) is identifiable up to a subspace-wise invertible transformation and a subspace-wise permutation.
\end{proposition}

==> sections/AAAI_2025/03-pre.tex <==
% In this section, we introduce notation expressing latent causal mechanisms. We also 
We formalize \textit{observed sources as auxiliaries} in terms of nonlinear ICA and CRL to construct our problem setting. 
% \subsection{Notation}
%
We use upper case letters for random variables or vectors, and lower case for their assignments.
Bold letters represent a set of random variables or random variables which is not a singleton.
% We represent bold letters for random vectors or vector functions. The opposite case represents a scalar random variable or scalar function. 
% We also employ upper case letters for a set of random vectors or random variables and an arbitrary transformation. 
We use $[d]$ to denote a set $\{1, 2, \cdots, d\}$.
% of the natural numbers from 1 to d.

\subsection{Observed Sources as Auxiliaries}
Let $\*{x} \in \mathbb{R}^m$ be an observation (e.g., image) generated from latent sources $\rvz \in \mathbb{R}^n$ with a mixing function $g$:
\begin{equation}\label{eqn1:generation}
    \rvx=g(\rvz),
\end{equation}
where $g$ is assumed to be an arbitrary invertible and smooth nonlinear function in the sense that its second-order derivatives exist.
By adopting a Bayesian network, we represent a data-generating process regarding latent sources as
\begin{equation}\label{eqn2:source dep}
    z_i = f_i(\Pa{z_i}, \epsilon_i), \quad \epsilon_i \sim p_{\epsilon_i}, 
\end{equation}
for all $i \in [n]$ 
where $\Pa{\cdot}$ represents parent nodes on a known causal graph $\mathcal{G}$ consisting of nodes $V$ and edges $E$.
Nonlinear ICA considers independent latent sources, i.e., 
\begin{equation}\label{eq:source-factorization-independent}
p(\rvz)=\prod_{i=1}^n p(z_i).
\end{equation}
% \paragraph{Nonlinear ICA} 
The primary goal is to recover inverse function $g^{-1}$ and the true independent components $\rvz=(z_1, \cdots, z_n)$ solely from observations. However, the model is known to be unidentifiable only with i.i.d samples \citep{10.1016/S0893-6080(98)00140-3}. This means that the mapping from observations to independent sources cannot be uniquely determined based solely on the assumption of mutually independent sources.

Accordingly, various conditions have been explored to address non-identifiability. The most widely used condition is independence given auxiliary observable variables $\rvu$, i.e., 
\begin{equation}\label{eq:source-factorization-independent-auxiliary}
p(\rvz\mid \rvu)=\prod_{i=1}^n p(z_i\mid \rvu),
\end{equation}
% $z_i \Perp z_j \mid \rvu$,
where $\rvu$
% The auxiliary variable $\rvu$ 
can be a class label, time index, or historical information \citep{pmlr-v89-hyvarinen19a}. 
Fig.~\ref{fig1:graph_a} illustrates a data generating process where $u$ is the observable and $\rvz=(z_1, z_2, z_3, z_4)$ is the latent sources that generates the observation.
However, they rely on the critical assumption that the auxiliary variable does not have a direct influence to the observation $\rvx$ to establish identifiability.

In this work, we consider a more generalized setup where the sources $\rvz$ could have arbitrary dependencies expressed by directed acyclic graph $\mathcal{G}$ and the arbitrary subset of the sources $\rvz_o \subset \rvz$ are observable. 
%For example, in Fig.~\ref{fig2:graph_b}, $z_5$ is observable where sources $\rvz$ have dependencies. Here, the observable variable $z_5$, along with other unobserved latent sources, generates the observation $\rvx$.
Note that CRL also aims to recover the latent sources with arbitrary dependencies, but it remains unclear how to leverage observed sources. We will discuss related works in nonlinear ICA and CRL in Sec.~\ref{sec:related-work}.

%%%%%%%%%%
To deal with the dependence between sources, we partition the latent sources into conditionally independent sets, 
% $Z_D =  \cup_{i=1}^{d} Z_{c_{i}}=(z_1,\dots,z_n)$ where variables in $Z_D$ do not need to be independent. 
$\rvz_{c_{i}} (i=1,...,d)$ where $\cup_{i=1}^{d} \rvz_{c_{i}} = \{z_1,\dots,z_n\}$. Thus, Eq.~\ref{eq:source-factorization-independent-auxiliary} can be restated in the context of observed sources as auxiliaries:
% It enables a more general formulation of Eq.~\ref{eq:source-factorization-independent} as \citet{zheng2023generalizing}:
% \begin{equation}\label{eq:source-factorization-zheng}
% p_{\rvz | \rvu}(\rvz | \rvu) = \prod_{i=1}^{n_i} p_{z_i}(z_i) \prod_{j=1}^{d} p_{\rvz_{c_j}| \rvu}(\rvz_{c_j}| \rvu).
% \end{equation}
% where $n_i$ is the number of mutually independent sources. \citet{zheng2023generalizing} partition all the sources into a set of mutually independent sources $\rvz_I$ and a set of variables in which do not need to be independent $\rvz_D = \cup_{i=1}^{d} \rvz_{c_{i}}$. 
% In Eq.~\ref{eq:source-factorization-partial}, we further generalize Eq.~\ref{eq:source-factorization-zheng} into the setting with observed sources, which includes Eq.~\ref{eq:source-factorization-zheng} as a special case in that $\rvu$ is independent from DGP.
\begin{equation}\label{eq:source-factorization-partial}
p_{\rvz_{o^-} \mid \rvz_o}(\rvz_{o^-} \mid \rvz_o) =  \prod_{j=1}^{d} p_{\rvz_{c_j}\mid \rvz_o}(\rvz_{c_j}\mid  \rvz_o).
\end{equation}
where $\rvz_o$ is observed sources and $\rvz_{o^-}$ is unobserved sources.
%%%%%%%%%%%%%%%%%%%%%%%%%

However, we do not consider the case where $\rvz_o $ is an empty set (i.e., an empty latent graph, without auxiliary variables), as this scenario requires additional assumptions such as structural sparsity for identifiability \citep{zheng2023generalizing}.

\begin{comment}
% There is also research on substituting auxiliary variables, such as assuming a Gaussian mixture distribution \citep{kivva2022identifiability} or structural sparsity \citep{zhang2024causal}.
% \begin{equation}
% p_{\rvz | \rvu}(\rvz | \rvu) = \prod_{i=1}^{n_i} p_{z_i}(z_i) \prod_{j=c_1}^{c_d} p_{\rvz_{c_j}| \rvu}(\rvz_{c_j}| \rvu).
% \end{equation}

Nonlinear ICA is a special case of CRL, which aims to recover the latent sources in a more generalized setting that the sources are not independent.
Thus, CRL requires stronger conditions to guarantee identifiability, such as sparsity assumption or the additional interventional data. Details of existing works of nonlinear ICA and CRL will be discussed in Sec.~\ref{sec:related-work}.

While there has been extensive research on CRL, the use of auxiliary variables in this setting has been less explored. This is because it is hard to satisfy the assumption of conditional independence on the setting of dependent sources. 
% Consider a data generating process (DGP) depicted in Fig.~\ref{fig1:graph_a}, which is the case of nonlinear ICA leveraging the auxiliary variable $u_1$.
% The auxiliary variable $u_1$ can make true sources independent. 
In contrast, on the DGP of CRL as Fig.~\ref{fig2:graph_b}, the observed $u_1$ cannot satisfy conditional independence for all sources.
\end{comment}




\input{figs/fig1}


\begin{comment}
By adopting a Structural Causal Model (SCM, \cite{reason:Pearl09a}), we represent a data-generating process regarding latent sources as
\begin{equation}\label{eqn2:source dep}
    z_i = f_i(\Pa{z_i}, \epsilon_i), \quad \epsilon_i \sim p_{\epsilon_i}, 
\end{equation}
for all $i \in [n]$ 
% where $\epsilon_i$ follows a noise distribution $p_{\epsilon_i}$ and 
where $\Pa{.}$ represents parent nodes on a latent causal graph $\mathcal{G}$ consisting of nodes $V$ and edges $E$.
\end{comment}

% The identifiability of the model Eq.~\ref{eq:source-factorization-zheng} is proved by Thm 4.3 of \citet{zheng2023generalizing}.
% % \begin{proposition}[\citet{zheng2023generalizing},~Thm~4.3]
% % \label{prop:identifiability-zheng-2023}
% %     123
% % \end{proposition}
% They address the undercomplete case of nonilinear ICA , where the dimension of the sources are smaller than the observations and there exists dependence between sources.

% We will address the issues that may arise from source dependence, specifically focusing on the latter term of Eq.~\ref{eq:source-factorization-zheng}. We will also deal with the setting of \textit{partially observable sources}, which can be viewed as more general model of  Eq.~\ref{eq:source-factorization-zheng} in terms of including the auxiliary variable in the mixing function $g$. The identifiability of this general setting in the \ref{appendix}

% In the Fig.~\ref{fig2:graph_b}, it is easy to find the most fine-grained (the easiest to identify) groups \citep{zheng2023generalizing}, i.e. ${(s_1),\,(s_2),\, (s_4,s_5)}$. However, if the number of all sources or observed sources are grown, it can be hard to find the proper latent grouping.

\subsection{Problem Formulation}\label{pre:problem}

Suppose a data generating process in Eq.~\ref{eqn1:generation} and Eq.~\ref{eqn2:source dep}. 
Our goal is to establish the identifiability of the independent latent sources (i.e., $\rvz_{c_i}$) up to certain subspace-wise invertible transformation and permutation, given the observations $\rvx$, observable sources $\rvz_o (\subseteq \rvz)$, and the latent Bayesian network $\mathcal{G}$ which encodes the conditional independence relationships between the latent sources as shown in Fig.~\ref{fig1}.

% Importantly, we do not rely on 
In contrast to previous works exploiting a specific factorization of the latent sources, e.g., Eq.~\ref{eq:source-factorization-independent} or Eq.~\ref{eq:source-factorization-zheng}, the knowledge of the latent Bayesian network $\mathcal{G}$ allows us to leverage diverse conditional independence relationships between the sources.
Importantly, the partition of the latent sources into subspaces $\rvz_{o^-}=\cup_i \rvz_{c_i}$ determines the \textit{degree} of the identifiability we could achieve (Thm. 4.3 of \citet{zheng2023generalizing}).
Therefore, it is crucial to capture the proper observable sources $\rvz_u\subseteq \rvz_o$ that entails fine-grained subspaces $\rvz_{c_j}$ mutually independent to each other conditioned on $\rvz_u$.

\paragraph{Motivating Examples}
%\label{sec:preliminary-example}
We illustrate the concept of a \textit{proper} auxiliary variable and \textit{fine-grained} subspaces through a representative example in Fig.~\ref{fig1}.

In Fig.~\ref{fig2:graph_b}, it is straightforward to find the most fine-grained conditionally independent groups, i.e. ${\{z_1\},\,\{z_2\},\, \{z_4,z_5\}}$. However, as the number of sources or observed sources increases, finding auxiliary variables that make the latent grouping fine-grained can become computationally challenging.

In addition, there is an another problem in exploiting auxiliary variables. Considering the case where the multiple sources are observed as Fig.~\ref{fig3:graph_c}, if all observed sources are conditioned, $z_1$ and $z_3$ cannot be disentangled. $z_2$ should not be conditioned to satisfy conditional independence. Although

It is true that dillema of which node to condition on typically arises in collider structures, but as the graph grows larger and more complex, the same node can act as a confounder for one group of nodes and as a collider for another. In such case, it becomes necessary to carefully choose which nodes to condition on in order to achieve optimal results.
% We can see that the graphical property of the observed auxiliary variables should be considered for the fine-grained recoverability in the causal representation learning. Therefore, we propose framework including graphical criterion for causal representation learning in the setup of partially observable sources. 

==> sections/AAAI_2025/04-method.tex <==

In this section, we establish identifiability in the presence of observable sources (Sec.~\ref{sec:method-identifiability}). Based on conditions for identifiability, we introduce a framework with a graphical criterion to effectively leverage auxiliary variables that makes the conditionally independent latents more fine-grained (Sec.~\ref{sec:method-selection}) and method to recover unobserved latents (Sec.~\ref{sec:method-architecture}).

\subsection{Identifiability}
\label{sec:method-identifiability}
We can consider existing approaches with auxiliary variables as the case that observed sources $\rvz_o$ do not have edges into the observations $\rvx$. (See Prop.~\ref{prop:auxiliary} in Appendix \ref{appx:id}.) 
To deal with problems that the observed sources $\rvz_o$ are included in the mixing function, we assume that the mixing function is constrained to a specific form as \citet{yang2022nonlinear}.
% We prove that we can identify sources in $Z_D$ up to a trivial indeterminacy with partially observed sources. There exists an invertible transformation $h_{c_i}$ such that $h_{c_i}(\rvz_{c_i}) = \hat{\rvz}_{c_i}$. We also generalize previous identifiability result of exploiting the auxiliary variables to the setting of partially observable sources. 
We adopt the proof of \citet{zheng2023generalizing} for identifiability with dependent sources.
% In \ref{eq:source-factorization-partial}, identifiability of the former term (i.e., about mutually independent sources) is not our focus. Its identifiability can be achieved as same as \citet{zheng2023generalizing} under assumption of Structural Sparsity. For theoretical guarantee of the identifiability on partially observable sources, we will present identifiability of latter term of \ref{eq:source-factorization-partial} (i.e., $n_i$ = 0) with its proof provided in Appendix \ref{appx:id}.
\input{proposition/proposition-partial-aaai}
Most prior works on CRL achieve identifiability by assuming the mixing function is fixed across environments. Under a common invertible mixing $g$, one can write the log-likelihood of the data under two domains and subtract them, causing the Jacobian log‐determinant terms to cancel (since the same $g$ applies in both cases). In such settings the latent distributions change across domains while $g$ remains invariant, so the log-determinant terms disappear when differencing log-likelihoods. 

In our setting, by contrast, the observed source (domain label) is used to index the mixing function, so $g$ varies with the source. As a result the usual cancellation does not occur and the standard identifiability proof breaks down. To address the problem, we constrain the mixing to be volume-preserving (i.e., $|\text{det}(\mathbf{J}_g(\rvz))| = 0$ everywhere). With the volume-preserving assumption on the mixing function, the Jacobian determinant remains constant at 1, making the log-determinant term equal to zero. Details of the proof are in Appendix \ref{appx:id}. 

% To address the determinant issues that arise from incorporating auxiliary variables in the mixing function, we introduced an additional assumption that constrains the mixing function to be volume-preserving. Details of the proof are in Appendix \ref{appx:id}. 
%In addition, it can be viewed as Independent Subspace Analysis (ISA) \citep{6789921,NIPS2006_20479c78}, which also covers ICA with the auxiliary variables under the condition of all $|\rvz_{c_i}| = 1$. 



% First, our framework select proper auxiliary variable among partially observed sources based on graphical criterion. 
% After the proper auxiliary variables are chosen, \ref{alg:inference} can find the most fine-grained subspaces which is conditionally independent between each other.

% Once the clusters are determined, we can efficiently identify true sources by reflecting the clustering results in the model design. We present effectiveness of our framework in \ref{sec:exp}.
% \paragraph{Selection Criterion for Observed Sources}



% \subsection{Partition of Graph}
\subsection{Selection on Observables}
\label{sec:method-selection}
According to the Prop.~\ref{prop:partial}, the conditional independence determines the number of recoverable sources in the identifiability of latent variables and our goal is first to capture mutually independent groups of nodes given observable sources and the known causal graph.
However, a naive approach of leveraging all observed sources might not capture conditional independence relationships, i.e., $z_1 \not \Perp z_3 \mid z_2, z_4$ in Fig.~\ref{fig3:graph_c}.
% In contrast, using only a subset of observable sources (i.e., $\{z_4\}$) leads to the conditional independence $z_1 \Perp z_3 \mid z_4$. 
It is necessary to capture a proper subset of observed sources that entails the most fine-grained groups of mutually independent sources, and ultimately, leads to the most granular identifiability.

Formally, we aim to discover a conditional independence structure that partition $\rvz_{o^-}$ into the most fine-grained subgroups such that:
\begin{equation}\label{eq:conditional-independence-cluster}
    \rvz_{c_i} \Perp \rvz_{c_j} \mid \rvz_u, \quad \text{for all } i\neq j,
\end{equation}
where $\rvz_u\subseteq \rvz_o$, $\cup_i \rvz_{c_i} \subseteq \rvz\setminus\rvz_o$, and $\rvz_{c_i}\cap \rvz_{c_j} = \emptyset$ for all $i\neq j$.
Importantly, satisfying a fine-grained conditional independence condition enables the identification of a greater number of latent variables. This ensures a more precise disentanglement of the underlying causal structure, leading to improved recoverability and manipulability of the true latent factors.

We propose a strategy that selects the most fine-grained conditionally independent groups of the latents with the minimum set of observed sources in Alg.~\ref{alg:selection}. The algorithm initializes a candidate set by including only nodes that act as confounders and excluding those that act solely as colliders, in order to account for nodes that may serve as both. The \textit{Partition} algorithm counts the number of groups that satisfy conditional independence by running \textit{Bayes-ball} \citep{10.5555/2074094.2074151} algorithm repeatedly. Finally, the algorithm outputs the conditioning set that results in the largest number of groups, i.e., the most fine-grained partitioning.

% We measure the \textit{degree} of identifiability for each subset of $\rvz_o$ based on the output of \ref{alg:iterative_bayes_ball} to find the most fine-grained partitioning.
% The \ref{alg:iterative_bayes_ball} examine the conditional independence of two node sets on the given the latent graph $\mathcal{G}$, conditioning set $C$, and observed set $O$. The dependent node set can change because the cluster is continuously changed by each iteration. Thus, \ref{alg:iterative_bayes_ball} repeatedly runs \textit{Bayes-ball} \citep{10.5555/2074094.2074151} algorithm until the result no longer changes and checks for conditional independence starting from all the nodes.
\input{algorithm/alg3_sc}
% \input{algorithm/alg2_gfc}
% Given a graph $\gG$, our goal is to discover mutually independent groups of nodes conditioned on partially observable sources $\rvz_o\subseteq \rvz$:
% \begin{equation}\label{eq:conditional-independence-cluster}
%     \rvz_{c_i} \Perp \rvz_{c_j} \mid \rvz_o, \quad \text{for all } i\neq j,
% \end{equation}
% where $\cup_i \rvz_{c_i} = \rvz\setminus\rvz_o$ and $\rvz_{c_i}\cap \rvz_{c_j} = \emptyset$ for all $i\neq j$.
% Recall that the granularity of such independent clusters determines the \textit{degree} of identifiability, we aim to find the fine-grained clusters that \ref{eq:conditional-independence-cluster} hold.
% i.e. which sources are included in $Z_{c_i}$. By leveraging graph $\mathcal{G}$, we can know the conditional independence between two nodes. 

 
 
% In \ref{eq:conditional-independence-cluster}, the observed sources are not restricted to a scalar value.
% The combination of nodes to be conditioned can vary.
% The granularity of the independent clusters can also vary by a combination of conditioning sets. We should consider which nodes are conditioned to achieve the \textit{better identifiability} among observed sources. The \textit{better identifiability} means achieving the most fine-grained identifiability using the minimum observed sources. 

\paragraph{Example}
Consider the latent graph in Fig.~\ref{fig3:graph_c}. Observed set $O = \{z_2, z_4\}$.
We will iterate all the subsets of $O$, i.e., $\{z_2\}, \{z_4\}, \{z_2,z_4\}$.\footnote{$\emptyset$ cannot be considered due to the identifiability  condition.}  Firstly, with conditioning set $\{z_2\}$, the partition process is as follows:
\begin{enumerate}
    \item Started from $z_1$, the \textit{result} contains $z_1$. 
    \item \textit{Bayes-ball} algorithm get input as $G,\{z_2\}$ and \textit{result}.
    \item In the \textit{Bayes-ball}, path from $z_1$ to $z_3$ through $z_2$ cannot be d-separated because $z_2$ works as collider.
    \item The path from $z_1$ to $z_3$ also cannot be d-separated.
    \item The \textit{result} is $ \{\{z_1,z_3\} \}$ except for observed source $z_2$.
\end{enumerate}
With conditioning set $\{z_4\}$, by following same process, the \textit{result} will be $\{ \{z_1\},\{z_3\} \}$. The conditioning set $\{z_2,z_4\}$ makes the result to be $\{ \{z_1,z_3\} \}$. Hence, the selection result will be $\{z_4\}$ for the most fine-grained conditionally independent latents. 

% Our goal is to find the most fine-grained conditionally independent subgroups to easily identify each $\*s_{D_i}$ and to select proper auxiliary variable that maximize recoverability. 
\subsection{Learning to Recover}
\label{sec:method-architecture}
To construct a representation that satisfies the identifiability conditions in Prop.~\ref{prop:partial}, we enforce volume preservation in the encoder by adopting  General Incompressible-flow Network (GIN) \citep{sorrenson2020disentanglementnonlinearicageneral} as our encoder. In addition to volume preservation, we also impose a graphical constraint via a structural neural network to preserve dependencies among latent variables that are not assumed to be independent, reflecting the known latent causal structure to strengthen disentanglement.
% We propose an architecture to recover unobserved sources with partially observed sources after the selection procedure. 
% We adopt General Incompressible-flow Network (GIN) \citep{sorrenson2020disentanglementnonlinearicageneral} as our encoder, which enforces the volume preservation of the mixing function $g$.
% To satisfy the identifiability condition that the mixing function has volume-preserving property as \ref{prop:partial}, we adopt General Incompressible-flow Network (GIN) \citep{sorrenson2020disentanglementnonlinearicageneral} as our encoder. 
%we additionally require taking into account that the information from the auxiliary variable is directly entangled with the observations

\paragraph{Volume-preservation} While GIN originally optimizes only the log-likelihood of the conditional distribution given the auxiliary variables, we factorize the log-likelihood of the distribution as follows:
\[
 \log p_{\hat{g}^{-1}}(\rvx) = \log p(\hat{\rvz}) =\log p(\rvz_u)+ \sum_i \log p(\hat{\rvz}_{u_{i}^-} \mid \rvz_u),
\]
where $\hat{\rvz}_{u_{i}^-}=\hat{\rvz}\setminus \hat{\rvz}_{u_{i}}$.
By factorizing the log-likelihood of the distribution, we can naturally address the issue that the information from the auxiliary variable is directly entangled with the observations. The preceding term will serve to absorb information about $\rvz_u$ from $\rvx$ while the latter term enforces the components of $\rvz_{u^-}$ to be independent given $\rvz_u$ by modeling them as a multivariate normal distribution with zero off-diagonal elements.

\paragraph{Graphical constraint} Besides, $\hat{\rvz}_{u^-}$ contain the information of sources that are observed but not selected (expressed as $\rvz_n$), i.e., $\hat{\rvz}_{u^-} = \{\hat{\rvz}_{o^-}, \hat{\rvz}_n\}$. We need to keep the relationship between $\hat{\rvz}_n$ and $\hat{\rvz}_{o^-}$ which is not independent (relationship between $z_2$ and ${z_1, z_3}$ in Fig.~\ref{fig3:graph_c}). 

To deal with this problem, we leverage the structural neural net to enforce the relationship between $\hat{\rvz}_{o^-}$ and $\hat{\rvz}_n$. A structural neural network is designed based on the latent graph $\mathcal{G}$ and not selected label $\rvz_n$.
Specifically, $\rvz_n$ is predicted by arbitrary dimensions of $\hat{\rvz}_{u^-}$ working as parents of $\rvz_n$. 
Since we do not know exactly which dimension of the representation corresponds to which true latent variable, we rely only on the number of parents of $\rvz_n$. For example, in Fig.~\ref{fig3:graph_c}, true $z_2$ is predicted by the certain dimension of the estimated representation given the other dimensions ($\hat{z}_1, \hat{z}_3$), naturally reflecting the causal structure. The full objective function is:
\begin{align}
\mathcal{L}(\theta) = \mathbb{E}_{(\rvx, \rvz_u, \rvz_n) \in \mathcal{D}} \Bigg[
    & \log p(\rvz_u) + \sum_i \log p(\hat{\rvz}_{u_{i}^-} \mid \rvz_u) \nonumber \\
    & + \log p(\rvz_n \mid \Pa{\rvz_n}) 
\Bigg].
\end{align}
% \begin{align}
% \mathcal{L} = 
%      \log p(\rvz_u) + \sum_i \log \\p(\hat{\rvz}_{u_{i}^-} \mid \rvz_u) 
%      + \log p(\rvz_n \mid \Pa{\rvz_n}) .
% \end{align}











==> sections/AAAI_2025/ReproducibilityChecklist.tex <==
\makeatletter
\@ifundefined{isChecklistMainFile}{
  % We are compiling a standalone document
  \newif\ifreproStandalone
  \reproStandalonetrue
}{
  % We are being \input into the main paper
  \newif\ifreproStandalone
  \reproStandalonefalse
}
\makeatother

% \ifreproStandalone
% \documentclass[letterpaper]{article}
% \usepackage[submission]{aaai2026}
% \setlength{\pdfpagewidth}{8.5in}
% \setlength{\pdfpageheight}{11in}
% \usepackage{times}
% \usepackage{helvet}
% \usepackage{courier}
% \usepackage{xcolor}
% \frenchspacing

% \begin{document}
% \fi
\setlength{\leftmargini}{20pt}
\makeatletter\def\@listi{\leftmargin\leftmargini \topsep .5em \parsep .5em \itemsep .5em}
\def\@listii{\leftmargin\leftmarginii \labelwidth\leftmarginii \advance\labelwidth-\labelsep \topsep .4em \parsep .4em \itemsep .4em}
\def\@listiii{\leftmargin\leftmarginiii \labelwidth\leftmarginiii \advance\labelwidth-\labelsep \topsep .4em \parsep .4em \itemsep .4em}\makeatother

\setcounter{secnumdepth}{0}
\renewcommand\thesubsection{\arabic{subsection}}
\renewcommand\labelenumi{\thesubsection.\arabic{enumi}}

\newcounter{checksubsection}
\newcounter{checkitem}[checksubsection]

\newcommand{\checksubsection}[1]{%
  \refstepcounter{checksubsection}%
  \paragraph{\arabic{checksubsection}. #1}%
  \setcounter{checkitem}{0}%
}

\newcommand{\checkitem}{%
  \refstepcounter{checkitem}%
  \item[\arabic{checksubsection}.\arabic{checkitem}.]%
}
\newcommand{\question}[2]{\normalcolor\checkitem #1 #2 \color{blue}}
\newcommand{\ifyespoints}[1]{\makebox[0pt][l]{\hspace{-15pt}\normalcolor #1}}

\section*{Reproducibility Checklist}

\vspace{1em}
\hrule
\vspace{1em}

\textbf{Instructions for Authors:}

This document outlines key aspects for assessing reproducibility. Please provide your input by editing this \texttt{.tex} file directly.

For each question (that applies), replace the ``Type your response here'' text with your answer.

\vspace{1em}
\noindent
\textbf{Example:} If a question appears as
%
\begin{center}
\noindent
\begin{minipage}{.9\linewidth}
\ttfamily\raggedright
\string\question \{Proofs of all novel claims are included\} \{(yes/partial/no)\} \\
Type your response here
\end{minipage}
\end{center}
you would change it to:
\begin{center}
\noindent
\begin{minipage}{.9\linewidth}
\ttfamily\raggedright
\string\question \{Proofs of all novel claims are included\} \{(yes/partial/no)\} \\
yes
\end{minipage}
\end{center}
%
Please make sure to:
\begin{itemize}\setlength{\itemsep}{.1em}
\item Replace ONLY the ``Type your response here'' text and nothing else.
\item Use one of the options listed for that question (e.g., \textbf{yes}, \textbf{no}, \textbf{partial}, or \textbf{NA}).
\item \textbf{Not} modify any other part of the \texttt{\string\question} command or any other lines in this document.\\
\end{itemize}

You can \texttt{\string\input} this .tex file right before \texttt{\string\end\{document\}} of your main file or compile it as a stand-alone document. Check the instructions on your conference's website to see if you will be asked to provide this checklist with your paper or separately.

\vspace{1em}
\hrule
\vspace{1em}

% The questions start here

\checksubsection{General Paper Structure}
\begin{itemize}

\question{Includes a conceptual outline and/or pseudocode description of AI methods introduced}{(yes/partial/no/NA)}
yes

\question{Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results}{(yes/no)}
yes

\question{Provides well-marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper}{(yes/no)}
yes

\end{itemize}
\checksubsection{Theoretical Contributions}
\begin{itemize}

\question{Does this paper make theoretical contributions?}{(yes/no)}
yes

	\ifyespoints{\vspace{1.2em}If yes, please address the following points:}
        \begin{itemize}
	
	\question{All assumptions and restrictions are stated clearly and formally}{(yes/partial/no)}
	yes

	\question{All novel claims are stated formally (e.g., in theorem statements)}{(yes/partial/no)}
	yes

	\question{Proofs of all novel claims are included}{(yes/partial/no)}
	yes

	\question{Proof sketches or intuitions are given for complex and/or novel results}{(yes/partial/no)}
	yes

	\question{Appropriate citations to theoretical tools used are given}{(yes/partial/no)}
	yes

	\question{All theoretical claims are demonstrated empirically to hold}{(yes/partial/no/NA)}
	yes

	\question{All experimental code used to eliminate or disprove claims is included}{(yes/no/NA)}
	NA
	
	\end{itemize}
\end{itemize}

\checksubsection{Dataset Usage}
\begin{itemize}

\question{Does this paper rely on one or more datasets?}{(yes/no)}
yes

\ifyespoints{If yes, please address the following points:}
\begin{itemize}

	\question{A motivation is given for why the experiments are conducted on the selected datasets}{(yes/partial/no/NA)}
	yes

	\question{All novel datasets introduced in this paper are included in a data appendix}{(yes/partial/no/NA)}
	yes

	\question{All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes}{(yes/partial/no/NA)}
	yes

	\question{All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations}{(yes/no/NA)}
	yes

	\question{All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available}{(yes/partial/no/NA)}
	yes

	\question{All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing}{(yes/partial/no/NA)}
	NA

\end{itemize}
\end{itemize}

\checksubsection{Computational Experiments}
\begin{itemize}

\question{Does this paper include computational experiments?}{(yes/no)}
yes

\ifyespoints{If yes, please address the following points:}
\begin{itemize}

	\question{This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting}{(yes/partial/no/NA)}
	yes

	\question{Any code required for pre-processing data is included in the appendix}{(yes/partial/no)}
	yes

	\question{All source code required for conducting and analyzing the experiments is included in a code appendix}{(yes/partial/no)}
	yes

	\question{All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes}{(yes/partial/no)}
	yes
        
	\question{All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from}{(yes/partial/no)}
	yes

	\question{If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results}{(yes/partial/no/NA)}
	yes

	\question{This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks}{(yes/partial/no)}
	partial

	\question{This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics}{(yes/partial/no)}
	yes

	\question{This paper states the number of algorithm runs used to compute each reported result}{(yes/no)}
	yes

	\question{Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information}{(yes/no)}
	yes

	\question{The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank)}{(yes/partial/no)}
	no

	\question{This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments}{(yes/partial/no/NA)}
	yes


\end{itemize}
\end{itemize}
\ifreproStandalone
% \end{document}
% \fi
